Learning Cross-hand Policies for High-DOF Reaching and Grasping

Reaching-and-grasping is a fundamental skill for robotic manipulation, but existing methods usually train models on a specific gripper and cannot be reused on another gripper. In this paper, we propose a novel method that can learn a unified policy model that can be easily transferred to different dexterous grippers. Our method consists of two stages: a gripper-agnostic policy model that predicts the displacements of pre-defined key points on the gripper, and a gripper-specific adaptation model that translates these displacements into adjustments for controlling the grippers' joints. The gripper state and interactions with objects are captured at the finger level using robust geometric representations, integrated with a transformer-based network to address variations in gripper morphology and geometry. In the experiments, we evaluate our method on several dexterous grippers and diverse objects, and the result shows that our method significantly outperforms the baseline methods. Pioneering the transfer of grasp policies across dexterous grippers, our method effectively demonstrates its potential for learning generalizable and transferable manipulation skills for various robotic hands.

==> figures/tab_partial.tex <==
\begin{table}[!t]\tiny
    \begin{center}
        \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
            \hline
            \multicolumn{1}{l|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{Schunk} & \multicolumn{2}{c|}{Schunk} & \multicolumn{2}{c|}{Mano} & \multicolumn{2}{c|}{Rutgers} & \multicolumn{2}{c}{Allegro}\\ \cline{2-11}
            %\textbf{Method}
            &  $S$  & $Q_1$ & $S$ & $Q_1$ & $S$ & $Q_1$ & $S$ & $Q_1$ & $S$ & $Q_1$\\ \hline
            Complete & 71.3$\%$ & 0.169 & 65.3$\%$ & 0.167 & 65.2$\%$ &	0.167 & 54.8$\%$ &	0.147 & 55.0$\%$ &	0.133\\ \hline 
            Partial & 67.3$\%$ & 0.182 & 58.6 $\%$ & 0.207 & 62.4$\%$ & 0.184 & 57.1$\%$ &	0.166 & 46.2$\%$ &	0.155\\ \hline
        \end{tabular}
    \end{center}
    \caption{
        Comparison results of our method under partial and complete observation
        settings.
    }
    \label{tab:partial}
\end{table}

==> figures/tab_update.tex <==
\begin{table}[!t]%
	\caption{
		The comparison among different adaptation models. "Online/Offline" refers to the source of training data.
		"1k/10k/50k/100k" refers to the model update number. We report success rates of the final grasps as well as the average generalized Q1 values
		among successful grasps.
	}
	\label{tab:comparation}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l|l|l|l|l|l}
				\hline
                \multicolumn{1}{l|}{\multirow{2}{*}{}} & \multicolumn{4}{c|}{Online} & \multicolumn{1}{c}{Offline} \\ \cline{2-6}
				\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{1k} & \multicolumn{1}{l|}{10k} & \multicolumn{1}{l|}{50k} & \multicolumn{1}{l|}{100k} & \multicolumn{1}{l}{50k} \\ \hline
				Generalized Q1  & 0.135 & 0.143 & 0.155 & 0.157 & 0.107 \\ \hline
                Success Rate & 26.5\% & 27.5\% & 38.8\% & 36.8\% & 6.1\%  \\ \hline
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/teaser.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.48\textwidth,]{images/banner.pdf}
    \caption {We propose a two-stage hierarchical model framework for cross-gripper reaching-and-grasping policy transfer. With gripper-agnostic representation, the policy learned on ShandowHand can be easily reused in 
    Rutgers Hand and Allegro hand by training a lightweight adaptation model}
    \label{fig:teaser}
\end{figure}

==> figures/update.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.36\textwidth]{images/update.pdf}
\caption{The Line graph of the loss function and success rate versus update times of the network.}
\label{fig:update}
\end{figure}
